Effective Cache Apportioning for Performance Isolation Under Compiler Guidance

With a growing number of cores in modern high-performance servers, effective sharing of the last level cache (LLC) is more critical than ever. The primary agenda of such systems is to maximize performance by efficiently supporting multi-tenancy of diverse workloads. However, this could be particularly challenging to achieve in practice, because modern workloads exhibit dynamic phase behaviour, which causes their cache requirements & sensitivities to vary at finer granularities during execution. Unfortunately, existing systems are oblivious to the application phase behavior, and are unable to detect and react quickly enough to these rapidly changing cache requirements, often incurring significant performance degradation. In this paper, we propose Com-CAS, a new apportioning system that provides dynamic cache allocations for co-executing applications. Com-CAS differs from the existing cache partitioning systems by adapting to the dynamic cache requirements of applications just-in-time, as opposed to reacting, without any hardware modifications. The front-end of Com-CAS consists of compiler-analysis equipped with machine learning mechanisms to predict cache requirements, while the back-end consists of proactive scheduler that dynamically apportions LLC amongst co-executing applications leveraging Intel Cache Allocation Technology (CAT). Com-CAS's partitioning scheme utilizes the compiler-generated information across finer granularities to predict the rapidly changing dynamic application behaviors, while simultaneously maintaining data locality. Our experiments show that Com-CAS improves average weighted throughput by 15% over unpartitioned cache system, and outperforms state-of-the-art partitioning system KPart by 20%, while maintaining the worst individual application completion time degradation to meet various Service-Level Agreement (SLA) requirements.

==> acmart/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> texes/intelcat.tex <==
\section{Probes Hoisting: Handling Recursive Calls}
For recursive functions, we do not hoist the probe calls outside the function call. This is because the loop-nest in a given recursive function-call is likely to be called with different iterations(trip-count), as the surrounding function is invoked with different input parameters. In short, caller-side hoisting is only done when the one does not enter Strongly-connected-component (SCC) through a caller-callee call edge.

==> texes/reuse.tex <==
\section{Reuse Behavior Example}

Fig. \ref{fig:code3} shows an example of how SRD can be leveraged to classify data-reuse behaviour of loop nests.

\begin{figure}[htp]
\centerline{\includegraphics[width=0.9\linewidth]{figs/SRD.jpg}}
\caption{Classifying Reuse Behaviour in a Loop Nest}
\label{fig:code3}
%\vspace{-10pt}
\end{figure}

The loop-nest shown in the above example has statements $S_1$ \& $S_2$, which have potential reuse of array \textit{A} \& statement $S_3$ has potential reuse of array \textit{B} among iterations of outer-loop. Statement $S_2$ reads a memory location which is re-read by $S_1$ after two iterations of I-loop. However, since every iteration of I-loop comes with \textit{N} intermediate iterations of statement $S_3$ from the inner-loop, thus SRD between two same accesses of $A[i]$ from $S_1$ \& $S_2$ will be $2 * N$. Similarly, each access to array \textit{B} from $S_3$ is repeated after every iteration of outer-loop, which makes the SRD equal to $M$. Since $M >> N$, the SRD from $S_1$ \& $S_2$ is insignificant and classified as \textit{streaming}, while the SRD from $S_3$ classifies the inner-loop as \textit{reuse}. In other words, for large reuse distances such as in $S_3$, sufficiently large cache resources must be allocated so that the reused data will be found in the cache whereas, even for very small cache resources the data which is reused only after a couple of iterations will be found in the cache. Overall, the entire loop-nest is classified as \textit{reuse} due to a significant \textit{reuse} component in $S_3$.

==> texes/suppl_eval.tex <==
\section{Supplemental Evaluation}
In this section, we will describe the additional components of our evaluation of Com-CAS. This includes justification of selecting specific benchmark suites (\S \ref{app:ben}), throughput evaluation on popular cache-insensitive SPEC 2017 (\S \ref{app:spec_thr}) and additional loop attribute prediction accuracy figures (\S \ref{app:accfig}).   

\subsection{Appropriate Benchmark Selection}
\label{app:ben}
To obtain the appropriate benchmarks suites for our experiments, we performed a study which measured the performance-sensitivity factor ($\alpha$). We found that \textbf{GAP} Benchmark Suite \cite{beamer2015gap}, \textbf{Rodinia} \cite{che2009rodinia} and \textbf{PolyBench} Suite \cite{pouchet2012polybench} have the maximum $\alpha$. These benchmarks represent memory-reuse heavy workloads from machine learning, data and graph analytics, etc, i.e domains that typically require multi-tenant execution environment \cite{amvrosiadis2018diversity}. In particular, these benchmarks exhibit intensive computations \& memory accesses in nested-loops, which usually constitutes the application bottleneck.  

In particular, we found that the SPEC 2017 Benchmark has extremely low values of $\alpha$, i.e only 5 individual benchmarks had $\alpha > 0$. Even among these 5 benchmarks, the individual $alpha$-values were $\leq 5$. As a reference, benchmarks in Polybench has $\alpha$-values as high as 80. This result is also ratified by the cache-sensitivity study performed in \cite{cook2013hardware}, which also concludes that SPEC 2017 is mostly cache-insensitive. Regardless, we added SPEC 2017 as a part of our supplemental evaluation for the sake of completeness. Table \ref{tab:ben} shows the final benchmarks used for our evaluation. From Polybench, we excluded benchmarks that had insignificant execution time $(\le 20 sec)$ since it makes the results non-repeatable.

\begin{table}[htbp]
\caption{List of Benchmarks used for evaluation}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|}
\hline
\textbf{Suite} & \textbf{Benchmarks} & \textbf{Input} \\ \hline
Polybench & \begin{tabular}[c]{@{}l@{}}Lu Correlation Covariance Gemm Symm Syr2k\\ Cholesky Trmm 2mm 3mm Doitgen Floyd-Warshall\\ Fdtd-2d Heat-3d Jacobi-2d, Seidel-2d\\ Nussinov Gramschimdt Syrk Adi Ludcmp\end{tabular} & \begin{tabular}[c]{@{}l@{}}MINI, STANDARD,\\ LARGE (Training)\\ EXTRALARGE \\ (Testing)\end{tabular} \\ \hline
GAP & BC CC CC\_SV TC PR SSSP BFS & \begin{tabular}[c]{@{}l@{}}Uniform Random\\ Graph (Train - $2^{22}$ nodes, \\ Test - $2^{24}$ nodes)\end{tabular} \\ \hline
Rodinia & \begin{tabular}[c]{@{}l@{}}Backprop LU Heartwall CFD  Hotspot Srad \\ Particlefilter Streamcluster\end{tabular} & \begin{tabular}[c]{@{}l@{}}Default Inputs (Train)\\ Customized Inputs (Test)\end{tabular} \\ \hline
SPEC 2017 & \begin{tabular}[c]{@{}l@{}}505.mcf\_r,  508.namd\_r, 510.parest\_r,  511.povray\_r, \\ 519.lbm\_r, 520.omnetpp\_r, 523.xalancbmk\_r, \\ 531.deepsjeng\_r, 538.imagick\_r, 541.leela\_r,\\ 544.nab\_r, 557.xz\_r\end{tabular} & \begin{tabular}[c]{@{}l@{}}SPEC\_ref, SPEC\_train (training)\\ SPEC\_test (testing)\end{tabular} \\ \hline
\end{tabular}}
\label{tab:ben}
\end{table}

\textbf{Mix Composition}: In the current evaluation, we don’t explicitly mix applications from different benchmarks suites. The reason for this is that the “mix-variability” is determined by the individual $\alpha$ value of a benchmark. In the individual benchmark suites, the $\alpha$ value ranged from 0 to ~80 for different benchmarks. Thus, while constructing the workload mixes, we ensure that different combinations of $\alpha$ value are included, resulting in three different workload categories.

\textbf{Reasoning about different workload mixes}: Different workload mixes can lead to different performances. However, we observed that performance gains are generally uniform across a particular mix category (light/medium/heavy). Thus, we can reason about the performance of an unknown workload mix by determining whether it’s a light/medium/heavy mix (by observing the $\alpha$ values), and then estimating the its performance gain accordingly.

\textbf{Non-Beneficial Applications}: In a real-life multi-execution environment, the incoming applications can be a mix of both cache-sensitive and cache-insensitive processes. Therefore, in evaluation, we accommodated such scenarios by categorizing the workload mixes as light (non-beneficial applications), medium and heavy. For light-mixes, the probe overheads do not degrade the overall performance, as evidenced by mixes from SPEC2017, which is mostly cache-insensitive. As a result, no ahead of time analysis is required to determine beneficial applications.

\subsection{Throughput Comparison on SPEC 2017}
Fig. \ref{spec_thr} summarizes our results on SPEC 2017 benchmarks. We created six mixes from this benchmark suite, each of which included benchmarks with $\alpha > 1$. We found that large mixes that had the highest $\alpha$ obtained the maximum throughput improvement.   
\label{app:spec_thr}
\begin{figure*}[!htbp]
\centerline{\includegraphics[width=1.0\linewidth]{figs/spec_thr.jpg}}
%\vspace{-0.08in}
\caption{Throughput improvement across SPEC 2017 Benchmarks between for KPart and Perf-Counter Baselines}
\label{spec_thr}
\end{figure*}


\subsection{Loop Attribute Graphs}
\label{app:accfig}
Fig. \ref{acc_graph} shows the probe prediction accuracy of loop timing. 

\begin{figure}[h]
\centerline{\includegraphics[width=1.0\linewidth]{figs/acc.png}}
\caption{Loop Timing Accuracy}
\label{acc_graph}
\end{figure}

%\begin{figure*}[h]
%\centerline{\includegraphics[width=1.0\linewidth]{figs/acc_merged.jpg}}
%\caption{Loop Timing \& Footprint Accuracy}
%\label{acc_graph}
%\end{figure*}
